Unsupervised Domain Expansion for Visual Categorization

Expanding visual categorization into a novel domain without the need of extra annotation has been a long-term interest for multimedia intelligence. Previously, this challenge has been approached by unsupervised domain adaptation (UDA). Given labeled data from a source domain and unlabeled data from a target domain, UDA seeks for a deep representation that is both discriminative and domain-invariant. While UDA focuses on the target domain, we argue that the performance on both source and target domains matters, as in practice which domain a test example comes from is unknown. In this paper we extend UDA by proposing a new task called unsupervised domain expansion (UDE), which aims to adapt a deep model for the target domain with its unlabeled data, meanwhile maintaining the model's performance on the source domain. We propose Knowledge Distillation Domain Expansion (KDDE) as a general method for the UDE task. Its domain-adaptation module can be instantiated with any existing model. We develop a knowledge distillation based learning mechanism, enabling KDDE to optimize a single objective wherein the source and target domains are equally treated. Extensive experiments on two major benchmarks, i.e., Office-Home and DomainNet, show that KDDE compares favorably against four competitive baselines, i.e., DDC, DANN, DAAN, and CDAN, for both UDA and UDE tasks. Our study also reveals that the current UDA models improve their performance on the target domain at the cost of noticeable performance loss on the source domain.

==> eval-toy.tex <==
\subsection{Experiments on Toy Data} \label{ssec:exp-toy}

To demonstrate the efficacy of our method, we design a concentric circles problem.
In this experiment, we will compare the decision boundaries of source-domain model, DA model and KDDE model.

% \subsubsection{Setup}
\textbf{Dataset.}
As shown in Figure \ref{fig:circles}, the plus signs indicate the positive class, the minus signs indicate the negative class.
The positive class contains 100 samples, and the negative class contains 300 samples.
Unlabeled target domain samples indicated by gray circle dots are generated by shifting horizontally the distribution of source domain samples 0.4 unit distance. All samplers are generated with scikit-learn\cite{scikit}.

\textbf{Implementation.}
The concentric circles problem is a 2-dimension classification problem.
All three models consist of a backbone and a classifier, while the DA model contains a discriminator in addition.
We use the multi-layer perceptron~(MLP) as backbone.
The backbones of the three models are the same network architecture that is a five-layer perceptron, of which each hidden layer contains 32 neurons followed by a batch normalization and a ReLU activation. 
The disciminator of the DA model is a three-layer perceptron whose hidden layer contains 32 neurons. 
To emphasize the effect of DA model, the coefficiient of adversarial domain adaptation loss $\lambda$ is set as 10.
To do domain expansion, we use the MLP trained with only source data as source-domain model and use the DA model as target-domain model, and then ditill them into a single KDDE model.

\begin{figure}[tbh!]
	\centering
	\includegraphics[width=\columnwidth]{diagrams/circles}
	\caption{\textbf{Concentric circles problem.} Source-domain model can make a better decision boundary for source domain samples, but can't distinguish target domain samples, while domain adaptation model does the opposite. KDDE model works best for categorizing all the source and target domain samples.}
	\label{fig:circles}
\end{figure}
%Blue "+"s, red "-"s and dots indicate source domain positive samples, source domain negative samples and target domian samples respectively. Three types of line indicate three models.
\textbf{Results.}
The dot, dashed and full lines are decision boundaries derived by source-domain model, DA model and KDDE model respectively. 
We observe that the source-domain model can classify source domain samples perfectly, but failing at target domain samples.
The DA model improve the performance on the target domain, however the performance on the source domain degrades.
We can see that some negative source samples at the left side are misclassified to positive class by the domain adaptation model.
Unlike domain adaptation, both domains are token into consideration in domain expansion task. 
By distilling the two models into a single one, we find that the KDDE model not only adapts to the target domain but also corrects the mistakes made by domain adaptation model.
This experiment shows effectiveness of our method in joint domain optimization over other methods.

